Angular distribution of $J/\psi$ decays in dimuon channel in 800 GeV proton-copper collisions

The anuglar distribution of $J/\psi$ decays in the $\mu^{+}\mu^{-}$ channel in 800 proton-copper collisions has been measured for $x_F$ > 0.25. The polarization parameter $\lambda$ is extracted in 1 GeV of $p_T$ and 0.1 of $x_F$ bins for two magnet configugrations with different acceptances. The data indicate that the $J/\psi$'s are produced with a slight transverse polarization at small $x_F$, which turns to longitudinal at $x_F$ > 0.6. No $p_T$ dependence of $\lambda$ is observed. Theoretical calculations are needed in order to interpret the measurements.

==> app2.tex <==
%auto-ignore
\chapter{Fitting the $J/\psi$ Peaks}
%\noindent {\bf APPENDIX B}

%\noindent {\bf Fitting the $J/\psi$ Peaks}\\

In this appendix the fitting of the $J/\psi$ peaks is presented. The di-muon
mass spectrum from each bin of $\cos \theta$, $p_T$, and $x_F$, are fitted to
a Gaussian plus a background function with $J/\psi$'s fitted to a Gaussian 
shape. The count of $J/\psi$'s in each bin was then calculated according to 
the output parameters of the Gaussian fit. Figure B1 to B42 show the fittings
from the ``SM12 = 2040 Amp'' data set, and Figure B43 to B84 show the fittings
from the ``SM12 = 2800 Amp'' data set.

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{10200_13-14-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $0<p_{t}<1$ and $0.25<x_{F}<0.35$]
{Fitting of the mass spectrum: $0<p_{t}<1$ and $0.25<x_{F}<0.35$. The 
backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2040 Ampere.}
\label{Fig:10200_13-14-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{10200_13-14-2.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $0<p_{t}<1$ and $0.25<x_{F}<0.35$]
{Fitting of the mass spectrum: $0<p_{t}<1$ and $0.25<x_{F}<0.35$.
 The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2040 Ampere.}
\label{Fig:10200_13-14-2}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{10300_13-14-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $0<p_{t}<1$ and $0.35<x_{F}<0.45$]
{Fitting of the mass spectrum: $0<p_{t}<1$ and $0.35<x_{F}<0.45$.
 The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2040 Ampere.}
\label{Fig:10300_13-14-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{10300_13-14-2.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $0<p_{t}<1$ and $0.35<x_{F}<0.45$]
{Fitting of the mass spectrum: $0<p_{t}<1$ and $0.35<x_{F}<0.45$.
 The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2040 Ampere.}
\label{Fig:10300_13-14-2}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{10400_13-14-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $0<p_{t}<1$ and $0.45<x_{F}<0.55$]
{Fitting of the mass spectrum: $0<p_{t}<1$ and $0.45<x_{F}<0.55$.
 The backgrounds were fitted to Kaplan
functions, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2040 Ampere.}
\label{Fig:10400_13-14-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{10400_13-14-2.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $0<p_{t}<1$ and $0.45<x_{F}<0.55$]
{Fitting of the mass spectrum: $0<p_{t}<1$ and $0.45<x_{F}<0.55$. 
The backgrounds were fitted to Kaplan
functions, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2040 Ampere.}
\label{Fig:10400_13-14-2}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{10500_13-14-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $0<p_{t}<1$ and $0.55<x_{F}<0.65$]
{Fitting of the mass spectrum: $0<p_{t}<1$ and $0.55<x_{F}<0.65$. 
The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2040 Ampere.}
\label{Fig:10500_13-14-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{10500_13-14-2.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $0<p_{t}<1$ and $0.55<x_{F}<0.65$]
{Fitting of the mass spectrum: $0<p_{t}<1$ and $0.55<x_{F}<0.65$. 
The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2040 Ampere.}
\label{Fig:10500_13-14-2}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{10600_13-14-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $0<p_{t}<1$ and $0.65<x_{F}<0.75$]
{Fitting of the mass spectrum: $0<p_{t}<1$ and $0.65<x_{F}<0.75$. 
The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2040 Ampere.}
\label{Fig:10600_13-14-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{10600_13-14-2.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $0<p_{t}<1$ and $0.65<x_{F}<0.75$]
{Fitting of the mass spectrum: $0<p_{t}<1$ and $0.65<x_{F}<0.75$. 
The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2040 Ampere.}
\label{Fig:10600_13-14-2}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{10700_13-14-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $0<p_{t}<1$ and $0.75<x_{F}<0.85$]
{Fitting of the mass spectrum: $0<p_{t}<1$ and $0.75<x_{F}<0.85$. 
The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2040 Ampere.}
\label{Fig:10700_13-14-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{10800_13-14-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $0<p_{t}<1$ and $0.85<x_{F}$]
{Fitting of the mass spectrum: $0<p_{t}<1$ and $0.85<x_{F}$. 
The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2040 Ampere.}
\label{Fig:10800_13-14-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{20200_13-14-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $1<p_{t}<2$ and $0.25<x_{F}<0.35$]
{Fitting of the mass spectrum: $1<p_{t}<2$ and $0.25<x_{F}<0.35$. 
The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2040 Ampere.}
\label{Fig:20200_13-14-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{20200_13-14-2.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $1<p_{t}<2$ and $0.25<x_{F}<0.35$]
{Fitting of the mass spectrum: $1<p_{t}<2$ and $0.25<x_{F}<0.35$. 
The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2040 Ampere.}
\label{Fig:20200_13-14-2}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{20300_13-14-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $1<p_{t}<2$ and $0.35<x_{F}<0.45$]
{Fitting of the mass spectrum: $1<p_{t}<2$ and $0.35<x_{F}<0.45$. 
The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2040 Ampere.}
\label{Fig:20300_13-14-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{20300_13-14-2.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $1<p_{t}<2$ and $0.35<x_{F}<0.45$]
{Fitting of the mass spectrum: $1<p_{t}<2$ and $0.35<x_{F}<0.45$. 
The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2040 Ampere.}
\label{Fig:20300_13-14-2}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{20400_13-14-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $1<p_{t}<2$ and $0.45<x_{F}<0.55$]
{Fitting of the mass spectrum: $1<p_{t}<2$ and $0.45<x_{F}<0.55$. 
The backgrounds were fitted to Kaplan
functions, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2040 Ampere.}
\label{Fig:20400_13-14-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{20400_13-14-2.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $1<p_{t}<2$ and $0.45<x_{F}<0.55$]
{Fitting of the mass spectrum: $1<p_{t}<2$ and $0.45<x_{F}<0.55$. 
The backgrounds were fitted to Kaplan
functions, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2040 Ampere.}
\label{Fig:20400_13-14-2}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{20500_13-14-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $1<p_{t}<2$ and $0.55<x_{F}<0.65$]
{Fitting of the mass spectrum: $1<p_{t}<2$ and $0.55<x_{F}<0.65$. 
The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2040 Ampere.}
\label{Fig:20500_13-14-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{20500_13-14-2.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $1<p_{t}<2$ and $0.55<x_{F}<0.65$]
{Fitting of the mass spectrum: $1<p_{t}<2$ and $0.55<x_{F}<0.65$. 
The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2040 Ampere.}
\label{Fig:20500_13-14-2}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{20600_13-14-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $1<p_{t}<2$ and $0.65<x_{F}<0.75$]
{Fitting of the mass spectrum: $1<p_{t}<2$ and $0.65<x_{F}<0.75$. 
The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2040 Ampere.}
\label{Fig:20600_13-14-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{20600_13-14-2.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $1<p_{t}<2$ and $0.65<x_{F}<0.75$]
{Fitting of the mass spectrum: $1<p_{t}<2$ and $0.65<x_{F}<0.75$. 
The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2040 Ampere.}
\label{Fig:20600_13-14-2}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{20700_13-14-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $1<p_{t}<2$ and $0.75<x_{F}<0.85$]
{Fitting of the mass spectrum: $1<p_{t}<2$ and $0.75<x_{F}<0.85$. 
The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2040 Ampere.}
\label{Fig:20700_13-14-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{30200_13-14-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $2<p_{t}<3$ and $0.25<x_{F}<0.35$]
{Fitting of the mass spectrum: $2<p_{t}<3$ and $0.25<x_{F}<0.35$. 
The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2040 Ampere.}
\label{Fig:30200_13-14-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{30200_13-14-2.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $2<p_{t}<3$ and $0.25<x_{F}<0.35$]
{Fitting of the mass spectrum: $2<p_{t}<3$ and $0.25<x_{F}<0.35$. 
The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2040 Ampere.}
\label{Fig:30200_13-14-2}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{30300_13-14-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $2<p_{t}<3$ and $0.35<x_{F}<0.45$]
{Fitting of the mass spectrum: $2<p_{t}<3$ and $0.35<x_{F}<0.45$. 
The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2040 Ampere.}
\label{Fig:30300_13-14-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{30300_13-14-2.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $2<p_{t}<3$ and $0.35<x_{F}<0.45$]
{Fitting of the mass spectrum: $2<p_{t}<3$ and $0.35<x_{F}<0.45$. 
The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2040 Ampere.}
\label{Fig:30300_13-14-2}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{30400_13-14-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $2<p_{t}<3$ and $0.45<x_{F}<0.55$]
{Fitting of the mass spectrum: $2<p_{t}<3$ and $0.45<x_{F}<0.55$. 
The backgrounds were fitted to Kaplan
functions, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2040 Ampere.}
\label{Fig:30400_13-14-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{30400_13-14-2.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $2<p_{t}<3$ and $0.45<x_{F}<0.55$]
{Fitting of the mass spectrum: $2<p_{t}<3$ and $0.45<x_{F}<0.55$. 
The backgrounds were fitted to Kaplan
functions, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2040 Ampere.}
\label{Fig:30400_13-14-2}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{30500_13-14-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $2<p_{t}<3$ and $0.55<x_{F}<0.65$]
{Fitting of the mass spectrum: $2<p_{t}<3$ and $0.55<x_{F}<0.65$. 
The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2040 Ampere.}
\label{Fig:30500_13-14-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{30500_13-14-2.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $2<p_{t}<3$ and $0.55<x_{F}<0.65$]
{Fitting of the mass spectrum: $2<p_{t}<3$ and $0.55<x_{F}<0.65$. 
The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2040 Ampere.}
\label{Fig:30500_13-14-2}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{30600_13-14-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $2<p_{t}<3$ and $0.65<x_{F}<0.75$]
{Fitting of the mass spectrum: $2<p_{t}<3$ and $0.65<x_{F}<0.75$. 
The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2040 Ampere.}
\label{Fig:30600_13-14-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{30600_13-14-2.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $2<p_{t}<3$ and $0.65<x_{F}<0.75$]
{Fitting of the mass spectrum: $2<p_{t}<3$ and $0.65<x_{F}<0.75$. 
The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2040 Ampere.}
\label{Fig:30600_13-14-2}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{30700_13-14-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $2<p_{t}<3$ and $0.75<x_{F}<0.85$]
{Fitting of the mass spectrum: $2<p_{t}<3$ and $0.65<x_{F}<0.75$. 
The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2040 Ampere.}
\label{Fig:30700_13-14-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{40200_13-14-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $3<p_{t}$ and $0.25<x_{F}<0.35$]
{Fitting of the mass spectrum: $3<p_{t}$ and $0.25<x_{F}<0.35$. 
The backgrounds were fitted to exponential
functions, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2040 Ampere.}
\label{Fig:40200_13-14-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{40200_13-14-2.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $3<p_{t}$ and $0.25<x_{F}<0.35$]
{Fitting of the mass spectrum: $3<p_{t}$ and $0.25<x_{F}<0.35$. 
The backgrounds were fitted to exponential
functions, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2040 Ampere.}
\label{Fig:40200_13-14-2}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{40300_13-14-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $3<p_{t}$ and $0.35<x_{F}<0.45$]
{Fitting of the mass spectrum: $3<p_{t}$ and $0.35<x_{F}<0.45$. 
The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2040 Ampere.}
\label{Fig:40300_13-14-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{40300_13-14-2.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $3<p_{t}$ and $0.35<x_{F}<0.45$]
{Fitting of the mass spectrum: $3<p_{t}$ and $0.35<x_{F}<0.45$. 
The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2040 Ampere.}
\label{Fig:40300_13-14-2}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{40400_13-14-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $3<p_{t}$ and $0.45<x_{F}<0.55$]
{Fitting of the mass spectrum: $3<p_{t}$ and $0.45<x_{F}<0.55$. 
The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2040 Ampere.}
\label{Fig:40400_13-14-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{40400_13-14-2.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $3<p_{t}$ and $0.45<x_{F}<0.55$]
{Fitting of the mass spectrum: $3<p_{t}$ and $0.45<x_{F}<0.55$. 
The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2040 Ampere.}
\label{Fig:40400_13-14-2}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{40500_13-14-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $3<p_{t}$ and $0.55<x_{F}<0.65$]
{Fitting of the mass spectrum: $3<p_{t}$ and $0.55<x_{F}<0.65$. 
The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2040 Ampere.}
\label{Fig:40500_13-14-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{40600_13-14-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $3<p_{t}$ and $0.65<x_{F}<0.75$]
{Fitting of the mass spectrum: $3<p_{t}$ and $0.65<x_{F}<0.75$. 
The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2040 Ampere.}
\label{Fig:40600_13-14-1}
\end{figure}


\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{10200_12-15-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $0<p_{t}<1$ and $0.25<x_{F}<0.35$]
{Fitting of the mass spectrum: $0<p_{t}<1$ and $0.25<x_{F}<0.35$.
 The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2800 Ampere.}
\label{Fig:10200_12-15-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{10200_12-15-2.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $0<p_{t}<1$ and $0.25<x_{F}<0.35$]
{Fitting of the mass spectrum: $0<p_{t}<1$ and $0.25<x_{F}<0.35$. 
The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2800 Ampere.}
\label{Fig:10200_12-15-2}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{10300_12-15-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $0<p_{t}<1$ and $0.35<x_{F}<0.45$]
{Fitting of the mass spectrum: $0<p_{t}<1$ and $0.35<x_{F}<0.45$.
 The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2800 Ampere.}
\label{Fig:10300_12-15-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{10300_12-15-2.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $0<p_{t}<1$ and $0.35<x_{F}<0.45$]
{Fitting of the mass spectrum: $0<p_{t}<1$ and $0.35<x_{F}<0.45$. 
The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2800 Ampere.}
\label{Fig:10300_12-15-2}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{10400_12-15-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $0<p_{t}<1$ and $0.45<x_{F}<0.55$]
{Fitting of the mass spectrum: $0<p_{t}<1$ and $0.45<x_{F}<0.55$.
 The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2800 Ampere.}
\label{Fig:10400_12-15-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{10400_12-15-2.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $0<p_{t}<1$ and $0.45<x_{F}<0.55$]
{Fitting of the mass spectrum: $0<p_{t}<1$ and $0.45<x_{F}<0.55$. 
The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2800 Ampere.}
\label{Fig:10400_12-15-2}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{10500_12-15-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $0<p_{t}<1$ and $0.55<x_{F}<0.65$]
{Fitting of the mass spectrum: $0<p_{t}<1$ and $0.55<x_{F}<0.65$.
 The backgrounds were fitted to Kaplan
functions, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2800 Ampere.}
\label{Fig:10500_12-15-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{10500_12-15-2.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $0<p_{t}<1$ and $0.55<x_{F}<0.65$]
{Fitting of the mass spectrum: $0<p_{t}<1$ and $0.55<x_{F}<0.65$.
 The backgrounds were fitted to Kaplan
functions, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2800 Ampere.}
\label{Fig:10500_12-15-2}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{10600_12-15-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $0<p_{t}<1$ and $0.65<x_{F}<0.75$]
{Fitting of the mass spectrum: $0<p_{t}<1$ and $0.65<x_{F}<0.75$.
 The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2800 Ampere.}
\label{Fig:10600_12-15-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{10600_12-15-2.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $0<p_{t}<1$ and $0.65<x_{F}<0.75$]
{Fitting of the mass spectrum: $0<p_{t}<1$ and $0.65<x_{F}<0.75$.
 The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2800 Ampere.}
\label{Fig:10600_12-15-2}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{10700_12-15-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $0<p_{t}<1$ and $0.75<x_{F}<0.85$]
{Fitting of the mass spectrum: $0<p_{t}<1$ and $0.75<x_{F}<0.85$.
 The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2800 Ampere.}
\label{Fig:10700_12-15-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{10800_12-15-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $0<p_{t}<1$ and $0.85<x_{F}$]
{Fitting of the mass spectrum: $0<p_{t}<1$ and $0.85<x_{F}$.
 The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2800 Ampere.}
\label{Fig:10800_12-15-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{20200_12-15-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $1<p_{t}<2$ and $0.25<x_{F}<0.35$]
{Fitting of the mass spectrum: $1<p_{t}<2$ and $0.25<x_{F}<0.35$. 
The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2800 Ampere.}
\label{Fig:20200_12-15-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{20200_12-15-2.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $1<p_{t}<2$ and $0.25<x_{F}<0.35$]
{Fitting of the mass spectrum: $1<p_{t}<2$ and $0.25<x_{F}<0.35$.
 The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2800 Ampere.}
\label{Fig:20200_12-15-2}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{20300_12-15-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $1<p_{t}<2$ and $0.35<x_{F}<0.45$]
{Fitting of the mass spectrum: $1<p_{t}<2$ and $0.35<x_{F}<0.45$.
 The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2800 Ampere.}
\label{Fig:20300_12-15-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{20300_12-15-2.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $1<p_{t}<2$ and $0.35<x_{F}<0.45$]
{Fitting of the mass spectrum: $1<p_{t}<2$ and $0.35<x_{F}<0.45$.
 The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2800 Ampere.}
\label{Fig:20300_12-15-2}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{20400_12-15-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $1<p_{t}<2$ and $0.45<x_{F}<0.55$]
{Fitting of the mass spectrum: $1<p_{t}<2$ and $0.45<x_{F}<0.55$.
 The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2800 Ampere.}
\label{Fig:20400_12-15-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{20400_12-15-2.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $1<p_{t}<2$ and $0.45<x_{F}<0.55$]
{Fitting of the mass spectrum: $1<p_{t}<2$ and $0.45<x_{F}<0.55$.
 The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2800 Ampere.}
\label{Fig:20400_12-15-2}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{20500_12-15-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $1<p_{t}<2$ and $0.55<x_{F}<0.65$]
{Fitting of the mass spectrum: $1<p_{t}<2$ and $0.55<x_{F}<0.65$.
 The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2800 Ampere.}
\label{Fig:20500_12-15-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{20500_12-15-2.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $1<p_{t}<2$ and $0.55<x_{F}<0.65$]
{Fitting of the mass spectrum: $1<p_{t}<2$ and $0.55<x_{F}<0.65$.
 The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2800 Ampere.}
\label{Fig:20500_12-15-2}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{20600_12-15-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $1<p_{t}<2$ and $0.65<x_{F}<0.75$]
{Fitting of the mass spectrum: $1<p_{t}<2$ and $0.65<x_{F}<0.75$.
 The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2800 Ampere.}
\label{Fig:20600_12-15-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{20600_12-15-2.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $1<p_{t}<2$ and $0.65<x_{F}<0.75$]
{Fitting of the mass spectrum: $1<p_{t}<2$ and $0.65<x_{F}<0.75$.
 The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2800 Ampere.}
\label{Fig:20600_12-15-2}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{20700_12-15-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $1<p_{t}<2$ and $0.75<x_{F}<0.85$]
{Fitting of the mass spectrum: $1<p_{t}<2$ and $0.75<x_{F}<0.85$.
 The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2800 Ampere.}
\label{Fig:20700_12-15-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{30200_12-15-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $2<p_{t}<3$ and $0.25<x_{F}<0.35$]
{Fitting of the mass spectrum: $2<p_{t}<3$ and $0.25<x_{F}<0.35$.
 The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2800 Ampere.}
\label{Fig:30200_12-15-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{30200_12-15-2.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $2<p_{t}<3$ and $0.25<x_{F}<0.35$]
{Fitting of the mass spectrum: $2<p_{t}<3$ and $0.25<x_{F}<0.35$.
 The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2800 Ampere.}
\label{Fig:30200_12-15-2}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{30300_12-15-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $2<p_{t}<3$ and $0.35<x_{F}<0.45$]
{Fitting of the mass spectrum: $2<p_{t}<3$ and $0.35<x_{F}<0.45$.
 The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2800 Ampere.}
\label{Fig:30300_12-15-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{30300_12-15-2.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $2<p_{t}<3$ and $0.35<x_{F}<0.45$]
{Fitting of the mass spectrum: $2<p_{t}<3$ and $0.35<x_{F}<0.45$.
 The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2800 Ampere.}
\label{Fig:30300_12-15-2}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{30400_12-15-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $2<p_{t}<3$ and $0.45<x_{F}<0.55$]
{Fitting of the mass spectrum: $2<p_{t}<3$ and $0.45<x_{F}<0.55$.
 The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2800 Ampere.}
\label{Fig:30400_12-15-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{30400_12-15-2.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $2<p_{t}<3$ and $0.45<x_{F}<0.55$]
{Fitting of the mass spectrum: $2<p_{t}<3$ and $0.45<x_{F}<0.55$.
 The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2800 Ampere.}
\label{Fig:30400_12-15-2}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{30500_12-15-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $2<p_{t}<3$ and $0.55<x_{F}<0.65$]
{Fitting of the mass spectrum: $2<p_{t}<3$ and $0.55<x_{F}<0.65$.
 The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2800 Ampere.}
\label{Fig:30500_12-15-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{30500_12-15-2.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $2<p_{t}<3$ and $0.55<x_{F}<0.65$]
{Fitting of the mass spectrum: $2<p_{t}<3$ and $0.55<x_{F}<0.65$.
 The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2800 Ampere.}
\label{Fig:30500_12-15-2}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{30600_12-15-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $2<p_{t}<3$ and $0.65<x_{F}<0.75$]
{Fitting of the mass spectrum: $2<p_{t}<3$ and $0.65<x_{F}<0.75$.
 The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2800 Ampere.}
\label{Fig:30600_12-15-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{30600_12-15-2.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $2<p_{t}<3$ and $0.65<x_{F}<0.75$]
{Fitting of the mass spectrum: $2<p_{t}<3$ and $0.65<x_{F}<0.75$.
 The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2800 Ampere.}
\label{Fig:30600_12-15-2}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{30700_12-15-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $2<p_{t}<3$ and $0.75<x_{F}<0.85$]
{Fitting of the mass spectrum: $2<p_{t}<3$ and $0.75<x_{F}<0.85$.
 The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2800 Ampere.}
\label{Fig:30700_12-15-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{40200_12-15-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $3<p_{t}$ and $0.25<x_{F}<0.35$]
{Fitting of the mass spectrum: $3<p_{t}$ and $0.25<x_{F}<0.35$.
 The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2800 Ampere.}
\label{Fig:40200_12-15-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{40200_12-15-2.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $3<p_{t}$ and $0.25<x_{F}<0.35$]
{Fitting of the mass spectrum: $3<p_{t}$ and $0.25<x_{F}<0.35$.
 The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2800 Ampere.}
\label{Fig:40200_12-15-2}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{40300_12-15-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $3<p_{t}$ and $0.35<x_{F}<0.45$]
{Fitting of the mass spectrum: $3<p_{t}$ and $0.35<x_{F}<0.45$.
 The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2800 Ampere.}
\label{Fig:40300_12-15-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{40300_12-15-2.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $3<p_{t}$ and $0.35<x_{F}<0.45$]
{Fitting of the mass spectrum: $3<p_{t}$ and $0.35<x_{F}<0.45$.
 The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2800 Ampere.}
\label{Fig:40300_12-15-2}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{40400_12-15-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $3<p_{t}$ and $0.45<x_{F}<0.55$]
{Fitting of the mass spectrum: $3<p_{t}$ and $0.45<x_{F}<0.55$.
 The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2800 Ampere.}
\label{Fig:40400_12-15-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{40400_12-15-2.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $3<p_{t}$ and $0.45<x_{F}<0.55$]
{Fitting of the mass spectrum: $3<p_{t}$ and $0.45<x_{F}<0.55$.
 The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2800 Ampere.}
\label{Fig:40400_12-15-2}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{40500_12-15-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $3<p_{t}$ and $0.55<x_{F}<0.65$]
{Fitting of the mass spectrum: $3<p_{t}$ and $0.55<x_{F}<0.65$.
 The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2800 Ampere.}
\label{Fig:40500_12-15-1}
\end{figure}

\clearpage

\begin{figure}
\begin{center}
\mbox{\epsfxsize=5.7in\epsfysize=6.5in\epsffile{40600_12-15-1.eps}}
\end{center}
\vspace*{+0.25in}
\caption[Fitting of the mass spectrum: $3<p_{t}$ and $0.65<x_{F}<0.75$]
{Fitting of the mass spectrum: $3<p_{t}$ and $0.65<x_{F}<0.75$.
 The backgrounds were fitted to second-order
polynomials, and the $J/\psi$'s were fitted to Gaussians. The $\cos \theta$ 
ranges are indicated under
each spectrum. The current of SM12 magnet was 2800 Ampere.}
\label{Fig:40600_12-15-1}
\end{figure}






